SWP: Microsecond Network SLOs Without Priorities

The increasing use of cloud computing for latency-sensitive applications has sparked renewed interest in providing tight bounds on network tail latency. Achieving this in practice at reasonable network utilization has proved elusive, due to a combination of highly bursty application demand, faster link speeds, and heavy-tailed message sizes. While priority scheduling can be used to reduce tail latency for some traffic, this comes at a cost of much worse delay behavior for all other traffic on the network. Most operators choose to run their networks at very low average utilization, despite the added cost, and yet still suffer poor tail behavior. This paper takes a different approach. We build a system, swp, to help operators (and network designers) to understand and control tail latency without relying on priority scheduling. As network workload changes, swp is designed to give real-time advice on the network switch configurations needed to maintain tail latency objectives for each traffic class. The core of swp is an efficient model for simulating the combined effect of traffic characteristics, end-to-end congestion control, and switch scheduling on service-level objectives (SLOs), along with an optimizer that adjusts switch-level scheduling weights assigned to each class. Using simulation across a diverse set of workloads with different SLOs, we show that to meet the same SLOs as swp provides, FIFO would require 65% greater link capacity, and 79% more for scenarios with tight SLOs on bursty traffic classes.

==> swpout.tex <==
\definecolor{burntorange}{rgb}{0.8, 0.33, 0.0}

\begin{Verbatim}[fontsize=\relsize{-2}, commandchars=\\\{\}]
  \textcolor{blue}{\textbf{\emph{Class}}} Foo

    \textcolor{purple}{\textbf{[SLI]} \textbf{|}} lat := mean of latencies
          \textcolor{purple}{\textbf{|}} \textcolor{red}{\textbf{=}} \textbf{18.948 µs}

    \textcolor{purple}{\textbf{[SLI]} \textbf{|}} sd := p99 of slowdowns where flowsizes : [:, 512_b]
          \textcolor{purple}{\textbf{|}} \textcolor{red}{\textbf{=}} \textbf{1.916x}

    \textcolor{burntorange}{\textbf{[SLO]} \textbf{|}} lat <= 12_us and sd < 2_x
          \textcolor{burntorange}{\textbf{|}} \textcolor{red}{\textbf{=}} \textcolor{red}{\textbf{False}}
          \textcolor{burntorange}{\textbf{|}}
          \textcolor{burntorange}{\textbf{|}} \textcolor{burntorange}{\textbf{\emph{The following constraints were not met:}}}
          \textcolor{burntorange}{\textbf{|}}   - \emph{lat <= 12_us}

\end{Verbatim}

==> todo.tex <==
\section{What we have}

Have I missed anything?

\begin{itemize}
    \item a model that is effective at predicting tail latency when there is a single bottleneck.
    \item An algorithm for determining hierarchical scheduling weights to achieve good tail latency with one bottleneck.
    \item A demonstration that weight tuning (with FIFO queues or fair queueing) is much better than priorities or FIFO with e2e congestion control for achieving good tail latency with bursty traffic and bursty flow lengths, even for multiple traffic classes
    \item  A demonstration that leaky bucket is not good at achieving good tail latency bounds (for bursty traffic/flow lengths).
    \item A model that predicts average? tail? latency for FIFO queues with one bottleneck for several e2e congestion control schemes (DCTCP and HPCC).  This is to simplify their behavior so that we don't need to model them in detail, using an oracle that allows the endpoint control to use lookback state.  (Still need to determine speedup relative to ns3 vs. our model of how DCTCP/HPCC works.) 
    \item A DSL for expressing SLO's on network traffic.
    \item code to turn a pdf of a traffic size distribution into a generative model.
\end{itemize}  

\section{Question}

A primary question is whether the single bottleneck model is good enough for predicting tail latency, or do we need a more sophisticated model. Ideas for this model: solve for each bottleneck separately, then add tail probabilities (this assumes a particular flow is slowed at only one bottleneck, rather than partially slowed across many).  Another approach is to simulate each path - for any pair of nodes, the behavior will be that of a path of links with different utilization and entering and leaving traffic. This will be more accurate, but has more options/configuration steps, although possibly symmetry can collapse most paths to one of a few models. Maybe the simpler model is close enough, or maybe the more complex model is only needed for those paths with nearly equally utilized, highly utilized links.

\section{What we need}

This is meant to be exhaustive - likely we can pare this down to what would be most important for a paper.
\begin{itemize}
    \item extend swp to take a topology (and link capacities) as input (not just a single bottleneck), and produce an estimate of tail latency, using whatever model is validated as being simplest and good enough
    \item Validate model. Mohammad's approach - generate a random traffic matrix (pairwise intensity between source/destination) that is admissible (doesn't exceed anyone's link capacity).  The distribution of traffic intensity between each pair is heavy tailed. Traffic on each path is heavy tailed and with the distribution of flow sizes from google (or a model of google). Simulate in ns3 as ground truth and compare to swp model, considering tail latency along each path (or type of path) separately.  The point is to characterize when the model works and when it doesn't. 
    \item performance metric of full data center swp vs. ns3 (how much of a speedup)
    \item evaluation: show the design space where tight latency bounds are possible, given different design options (e.g., with FIFO queues and e2e cc, with priority queues and e2e cc, with traffic classes and adjustable weights, with hierarchical FQ) and different workloads (more bursty/less bursty, higher/lower utilization, single bottleneck vs. clos topology, etc.) This quantifies how much you lose using weaker methods for SLO management like FIFO queues and e2e CC.
    \item Algorithm for collecting workload from one-way latencies for sampled RPC. How do we collect source/destination intensity/burstiness?  Can we estimate error implied by sampling - if we only observe 1:100 RPCs, how accurate will we be at estimating the true workload (even ignoring that the true workload might not be stochastic)?
    \item write an e2e cc that would be effective at keeping links full and buffers small with weighted fair queueing, or approximate wfq. If we don't want to explain bfc (and we don't, imo), then that's the obvious alternative and it will work reasonably well.
    \item gradient search optimization for traffic weights rather than brute force
    \item estimate error when workload is outside of estimated range; show that we can achieve bounds even in this case, given an assumption of the rate of workload divergence (by building in a tolerance for change in the model)
    \item enforcement: how do we detect when a traffic class is exceeding our measured CBE? 
    \item pricing: can we detect/charge if an app is byzantine?
    \item quantitative comparison against silo and not just qjump (for bursty workload)
    \item (eventual) Validation against (sampled?) real-world RPC trace. 
\end{itemize}


==> tyerror.tex <==
\begin{Verbatim}[fontsize=\relsize{-2}, commandchars=\\\{\}]
  \textbf{\textcolor{red}{error}: type mismatch: expected `Time`, got `Factor`}
    \textcolor{blue}{-->} foo.slo:13:8
     \textcolor{blue}{|}
  \textcolor{blue}{13 |} bar <= 5_x and baz < 2_x
     \textcolor{blue}{|}        \textcolor{red}{^^^}
\end{Verbatim}
